Tractable Conjunctive Queries over Static and Dynamic Relations

We investigate the evaluation of conjunctive queries over static and dynamic relations. While static relations are given as input and do not change, dynamic relations are subject to inserts and deletes. We characterise syntactically three classes of queries that admit constant update time and constant enumeration delay. We call such queries tractable. Depending on the class, the preprocessing time is linear, polynomial, or exponential (under data complexity, so the query size is constant). To decide whether a query is tractable, it does not suffice to analyse separately the sub-queries over the static relations and over the dynamic relations, respectively. Instead, we need to take the interaction between the static and the dynamic relations into account. Even when the sub-query over the dynamic relations is not tractable, the overall query can become tractable if the dynamic relations are sufficiently constrained by the static ones.

==> app_prelims.tex <==
\section{Further Preliminaries}
\label{app:prelims}
We recall some notions that were omitted in Section~\ref{sec:prelims}. 
We start with well-known width measure for queries.

\begin{definition}[Fractional Edge Cover~\cite{AtseriasGM13}]
\label{def:fractional_edge_cover}
Given a CQ $Q$ and $\calF \subseteq \vars(Q)$,    
a {\em fractional edge cover}
of $\calF$ is a solution 
$\boldsymbol{\lambda} = (\lambda_{R(\calX)})_{R(\calX) \in \atoms(Q)}$ to the following 
linear program: 
\begin{align*}
\text{minimize} & \TAB\sum_{R(\calX) \in\, \atoms(Q)} \lambda_{R(\calX)} && \\[3pt]
\text{subject to} &\TAB \sum_{R(\calX)\in\, \atoms(Q) \text{ s.t. } X \in \calX}\hspace{-0.5cm} \lambda_{R(\calX)} \geq 1 && \text{ for all } X \in \calF \text{ and } \\[3pt]
& \TAB\lambda_{R(\calX)} \in [0,1] && \text{ for all } R(\calX) \in \atoms(Q)
\end{align*}
The optimal objective value of the above program 
is called the {\em fractional edge cover number} of the variable set $\calF$ 
and is denoted as $\rho_{Q}^{\ast}(\calF)$.  
If $Q$ is clear from the context, we omit 
the index $Q$ and write $\rho^{\ast}(\calF)$. When all $Q$'s variables are considered, namely $\calF = \vars(Q)$, we write $\rho^*(Q)$.
For a database of size $N$, the result of a query $Q$ without bound variables can be computed in time 
$\bigO{N^{\rho^*(Q)}}$~\cite{Ngo:JACM:18}.
\end{definition}

\begin{definition}[Tree Decomposition]
\label{def:tree_decomposition}
A tree decomposition of a CQ $Q$ is a pair $(\calT, \chi)$, where $\calT$ is a tree with vertices $V(\calT)$ and $\chi: V(\calT) \rightarrow 2^{\vars(Q)}$ maps each node $t$ of the tree $\calT$ to a subset $\chi(t)$ of variables of $Q$ such that the following properties hold:
\begin{enumerate}
    \item for every atom $R(X) \in \atoms(Q)$, the schema $X$ is a subset of $\chi(t)$ for some $t \in V(\calT)$,
    \item for every variable $X \in \vars(Q)$, the set $\{t | X \in \chi(t)\}$ is a non-empty connected subtree of $\calT$. The sets $\chi(t)$ are called the bags of the tree decomposition.
\end{enumerate}
A tree decomposition is free-connex if it has a connected sub-tree
such that the union of the bags of this sub-tree are the free variables.
We use $TD(Q)$ to denote the set of free-connex tree decompositions of $Q$.
\end{definition}

\begin{definition}[Fractional Hypertree Width]
\label{def:factional_hypertree_width}
Given a CQ $Q$ and a free-connex tree decomposition $(\calT, \chi)$ of $Q$, the fractional hypertree width of $(\calT, \chi)$ and of $Q$ are defined 
as follows:
\begin{align*}
    w(\calT, \chi) & = \max_{t \in V(\calT)} \rho^*_Q(\chi(t))\\
    w(Q) & = \min_{(\calT, \chi) \in TD(Q)} w(\calT, \chi)
\end{align*}
%We call a tree decomposition $(\calT, \chi)$ of $Q$ optimal if $w(\calT, \chi) = w(Q)$.
\end{definition}

Next, we overview the widely believed complexity-theoretic conjectures.

\begin{definition}[Boolean Matrix Multiplication (BMM) Problem~\cite{BaganDG07}]
\label{def:BMM_problem}
Given two $n \times n$ Boolean matrices $A$ and $B$, represented as lists of their non-zero entries, the task is to output the product $AB$.
\end{definition}

\begin{conjecture}[BMM conjecture~\cite{BaganDG07}]
\label{conj:BMM}
The BMM problem cannot be solved in time $m^{1 + o(1)}$, where $m$ is the number of non-zero entries in $A$, $B$ and $AB$.
\end{conjecture}

\begin{definition}[Online Matrix-Vector Multiplication (OMv) Problem~\cite{Henzinger:OMv:2015}]
\label{def:OMV_problem}
We are given an $n \times n$ Boolean matrix $M$ and receive $n$ Boolean column vectors $v_1,\dots, v_n$ of size $n$, one by one. After seeing each vector $v_i$, the task is to output the product $Mv_i$ before seeing the next vector.
\end{definition}

\begin{conjecture}[OMv Conjecture~\cite{Henzinger:OMv:2015}]
\label{conj:OMV}
For any constant $\gamma > 0$, there is no algorithm that solves the 
OMv problem in time $\bigO{n^{3-\gamma}}$.
\end{conjecture}

\begin{definition}[Online Vector-Matrix-Vector Multiplication (OuMv) Problem~\cite{Henzinger:OMv:2015}]
\label{def:OuMV_problem}
We are given an $n \times n$ Boolean matrix $M$ and receive $n$ pairs of Boolean column vectors $(u_1, v_1),\dots, (u_n, v_n)$ of size $n$, one by one. 
% we multiply the matrix with two vectors, one from the left and one from the right
After seeing each pair of vectors $(u_i, v_i)$, the task is to output the product $u_iMv_i$ before seeing the next pair.
\end{definition}

The following OuMv conjecture is implied by the OMv conjecture.

\begin{conjecture}[OuMv Conjecture~\cite{Henzinger:OMv:2015}]
\label{conj:OuMV}
For any constant $\gamma > 0$, there is no algorithm that solves OuMv 
problem in time $\bigO{n^{3-\gamma}}$.
\end{conjecture}

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

==> results.tex <==
\section{Main Results}
\label{sec:results}
\ahmet{Section in progress.}














